Scalable Simulation of Realistic Volume Fraction Red Blood Cell Flows through Vascular Networks

High-resolution blood flow simulations have potential for developing better understanding biophysical phenomena at the microscale, such as vasodilation, vasoconstriction and overall vascular resistance. To this end, we present a scalable platform for the simulation of red blood cell (RBC) flows through complex capillaries by modeling the physical system as a viscous fluid with immersed deformable particles. We describe a parallel boundary integral equation solver for general elliptic partial differential equations, which we apply to Stokes flow through blood vessels. We also detail a parallel collision avoiding algorithm to ensure RBCs and the blood vessel remain contact-free. We have scaled our code on Stampede2 at the Texas Advanced Computing Center up to 34,816 cores. Our largest simulation enforces a contact-free state between four billion surface elements and solves for three billion degrees of freedom on one million RBCs and a blood vessel composed from two million patches.

==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler (default pdf)
##  $ make OUTOFSRC=no       #make in the same directory, otherwise inside ${BIULDDIR}
##
###

## user flags
PROJ     ?= $(notdir $(shell pwd))#defaults to dirname
OUTEXT   ?= pdf
SUMMARY  ?= grep -in --color=always "\(error\|warn\|warning\|repeated\|skipping\)"
POSTSUM  ?= awk '{ gsub("undefined", "\033[1;33m&\033[0m"); gsub("multiply defined", "\033[1;36m&\033[0m"); print }'
SYNC     ?= -synctex=1
OUTOFSRC ?= yes
BUILDDIR ?= ${_BUILDDIR}
TEMP_WC  = *.auxlock *-blx.bib *.bbl *.run.xml *.spl

ifeq ($(strip ${SCRATCH}),)
  _BUILDDIR = _build
else
  _BUILDDIR = ${SCRATCH}/$(strip ${PROJ})/_build
endif

ifeq ($(strip ${OUTOFSRC}),no)
  _BUILDDIR = ${CURDIR}
endif

## programs
LXX      ?= latexmk
PDFLATEX ?= pdflatex
LATEX	 ?= latex
BIBTEX	 ?= bibtex
DVI	 ?= dvipdf
PS	 ?= ps2pdf
MKDIR    ?= mkdir
OPEN     ?= open

## internal flag
LXFLAG 	 ?= -g -file-line-error -halt-on-error -shell-escape ${SYNC}
TEXFILES ?= $(shell ls -b *.tex *.bib)

ifeq (${OUTEXT},pdf)
  LXFLAG += -pdf
endif

BIBINPUTS:="..;${CURDIR};${BIBINPUTS};"
TEXINPUTS:="..;${CURDIR};${TEXINPUTS};;"
TRGS=${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})
export

all:${TRGS}

help:
	@head -14 ${MAKEFILE_LIST}

${BUILDDIR}:
	${MKDIR} -p ${BUILDDIR}
	${MKDIR} -p ${BUILDDIR}/figs

%.${OUTEXT}:${TEXFILES} ${BUILDDIR}
	@echo "building out of source in ${BUILDDIR} for $(notdir $*)"
	cd ${BUILDDIR} && ${LXX} ${LXFLAG} ${CURDIR}/$(addsuffix .tex, $(notdir $*))
	${SUMMARY} ${BUILDDIR}/*.log ${BUILDDIR}/*.blg | ${POSTSUM}

o: open
open:
	@echo "opening ${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})"
	@${OPEN} -a /Applications/TeX/TeXShop.app ${BUILDDIR}/$(addsuffix .${OUTEXT}, ${PROJ})

dir:
	@echo "${BUILDDIR}"

info:
	@echo "Build directory is ${BUILDDIR}"

archive:
	hg archive --include "*" --exclude "result_data" $(addsuffix .tgz, ${PROJ})

clean:
	@if [ ${BUILDDIR} -ef ${CURDIR} ]; then \
        ${LXX} -C ${LXFLAG} ${TRGS} && ${RM} ${TEMP_WC}; else \
        echo "${RM} -r ${BUILDDIR}" && ${RM} -r ${BUILDDIR}; \
	fi

.PHONY: clean open all

